Surprisal-Triggered Conditional Computation with Neural Networks

Autoregressive neural network models have been used successfully for sequence generation, feature extraction, and hypothesis scoring. This paper presents yet another use for these models: allocating more computation to more difficult inputs. In our model, an autoregressive model is used both to extract features and to predict observations in a stream of input observations. The surprisal of the input, measured as the negative log-likelihood of the current observation according to the autoregressive model, is used as a measure of input difficulty. This in turn determines whether a small, fast network, or a big, slow network, is used. Experiments on two speech recognition tasks show that our model can match the performance of a baseline in which the big network is always used with 15% fewer FLOPs.

==> appendices.tex <==
\clearpage
\normalsize
\section*{Appendix A: Effect of varying hyperparameters}
We re-ran the ablation experiment on TIMIT using three other neural architectures different from the one used in our main experiments, listed here in more concise PyTorch-like notation. For these models, the controller trained to have mean 0.65 for $p_{big}$, instead of 0.5. The results show that using surprisal for effort allocation at test time improves PER across different hyperparameter settings, and that the pre-net, post-net, and recurrent layers are not essential for the idea to work. Using different hyperparameters for the autoregressive model would also be worthwhile to explore, but as training it is time-consuming, we have restricted the autoregressive model to a single configuration.

% Model 1 Table
\begin{wraptable}{r}{10cm}
% \centering
\caption{Model 1 results for TIMIT.}
\label{model-1}
\begin{tabular}{cccc} %{llllll}
\toprule
\thead{Surprisal-based\\ during training?} & \thead{Surprisal-based\\ during testing?} & \thead{PER} & \thead{Avg. FLOPs\\per input}\\
\midrule
\xmark & \xmark     & 26.94\% $\pm$ 0.48\%  &  6.52M     \\ % 
\rowcolor[gray]{.75}\xmark  & \cmark  &  26.89\% $\pm$ 0.20\%   & 6.49M  \\ % 
\cmark & \xmark  &  28.86\% $\pm$ 0.31\%  &  6.52M     \\% 
\cmark & \cmark  & 27.51\% $\pm$ 0.39\%  & 6.49M   \\ % 
\midrule
\rowcolor[gray]{.75}\multicolumn{2}{c}{Small network only}   & 27.72\% $\pm$ 0.53\% &  \textbf{5.96M}  \\ % & 63.49 $\pm$ 0.26
\rowcolor[gray]{.75}\multicolumn{2}{c}{Big network only}  &  \textbf{26.75\%} $\pm$ 0.13\%  & 7.07M \\ % &  \textbf{61.94} $\pm$ 0.89 
\bottomrule
\end{tabular}
\end{wraptable}

% \vspace{0.5cm}
\textbf{Model 1:}

% \vspace{-0.125cm}
\textit{Pre-net:} \\
\texttt{Conv1D(length 11, 512 filters)\\
LeakyReLU(0.125)}

\textit{Small network:}\\
\texttt{Linear(512, 40)\\
LogSoftmax()}

\textit{Big network:}\\
\texttt{Linear(512, 2048)\\
LeakyReLU(0.125)\\
Linear(2048, 40)\\
LogSoftmax()}

\textit{Post-net:} (none)

% Model 2 Table
\begin{wraptable}{r}{9cm}
% \centering
\caption{Model 2 results for TIMIT.}
\label{model-2}
\begin{tabular}{cccc} %{llllll}
\toprule
\thead{Surprisal-based\\ during training?} & \thead{Surprisal-based\\ during testing?} & \thead{PER} & \thead{Avg. FLOPs\\per input}\\
\midrule
\xmark & \xmark     &  26.76\% $\pm$ 0.11\% &  6.52M     \\ % 
\rowcolor[gray]{.75}\xmark  & \cmark  & 26.30\% $\pm$ 0.36\% & 6.49M  \\ % 
\cmark & \xmark  &  28.16\% $\pm$ 0.27\%  & 6.52M \\% 
\cmark & \cmark  & 26.54\% $\pm$ 0.32\%  & 6.49M  \\ % 
\midrule
\rowcolor[gray]{.75}\multicolumn{2}{c}{Small network only}   &  27.60\% $\pm$ 0.60\% &  \textbf{5.96M}  \\ % & 63.49 $\pm$ 0.26
\rowcolor[gray]{.75}\multicolumn{2}{c}{Big network only}  & \textbf{25.91\%} $\pm$ 0.41\%   & 7.07M \\ % &  \textbf{61.94} $\pm$ 0.89 
\bottomrule
\end{tabular}
\end{wraptable}

\vspace{0.25cm}
\textbf{Model 2:}

Model 2 is the same as Model 1, except we add \texttt{Dropout(0.5)} to the end of the pre-net. (We found that the variants of Model 1 trained with surprisal easily overfit, which we believe happens because it is easier for the big and small networks to model either only surprising inputs or only unsurprising inputs separately than a mixture of both types.)


% Model 3 Table
\begin{wraptable}{r}{10cm}
% \centering
\caption{Model 3 results for TIMIT.}
\label{model-3}
\begin{tabular}{cccc}
\toprule
\thead{Surprisal-based\\ during training?} & \thead{Surprisal-based\\ during testing?} & \thead{PER} & \thead{Avg. FLOPs\\per input}\\
\midrule
\xmark & \xmark     &  32.30\% $\pm$ 0.66\%  &   4.62M    \\ % 
\xmark  & \cmark  &  31.14\% $\pm$ 0.54\%  & 4.54M   \\ % 
\cmark & \xmark  &  34.07\% $\pm$ 0.58\%   &  4.62M    \\% 
\rowcolor[gray]{.75}\cmark & \cmark  &  30.37\% $\pm$ 0.31\%  &  4.54M   \\ % 
\midrule
\rowcolor[gray]{.75}\multicolumn{2}{c}{Small network only}   & 35.47\% $\pm$ 0.68\%  &   \textbf{3.28M}  \\ 
\rowcolor[gray]{.75}\multicolumn{2}{c}{Big network only}  &  \textbf{28.04\%}  $\pm$ 0.55\%  & 5.96M \\ 
\bottomrule
\end{tabular}
\end{wraptable}

\vspace{0.25cm}
\textbf{Model 3:}

\textit{Pre-net:} (none)

\textit{Small network:}\\
\texttt{Dropout(0.5),\\
Conv1D(length 11, 40 filters)\\
LogSoftmax()}

\textit{Big network:}\\
\texttt{Dropout(0.5),\\
Conv1D(length 11, 512 filters)\\
LeakyReLU(0.125)\\
Linear(512, 40)\\
LogSoftmax()}

\textit{Post-net:} (none)


\clearpage
\section*{Appendix B: Effect of varying controller bias}

To investigate the effect of a mismatch between train time and test time further, we ran an experiment with Mini-LibriSpeech in which the bias parameter of the controller of models trained with surprisal is gradually increased from (average bias value learned when training the controller) to (that value $+$ 4) in uniform increments. This increases the probability of using the big network from what it was during training. 

The resulting sweep of mean test PERs with standard deviations is shown in Figure \ref{fig:sweep}. Using the big network more does decrease PER up to a point, but when the bias is increased to the point where the big network is always sampled, the conditional model does not attain the same PER as the model that only ever uses the big network during training and testing. In fact, PER begins to increase, which may be because the big network is exposed to a distribution of more unsurprising inputs than it was shown during training.

In general, though, always using the big network may not be expected to yield the best performance; using both the big and small networks at different times may have an ensemble effect, which may explain how the conditional models in our main experiments were able to slightly outperform the model using only the big network for TIMIT.

\begin{figure}[h]
    \centering
\hspace*{-0.5cm} 
    \begin{tikzpicture}[font=\fontsize{7}{7}\selectfont]
\begin{axis}[
    % ytick={, 26.3},
    legend style={at={(0.7,0.175)},anchor=north},
        height=5.5cm,
        width=7cm,
        xmin=-1.25,
        xmax=3,
        ymin=25.6,
        ymax=26,
        every axis plot/.append style={thick},
        xlabel=Controller bias,
        ylabel=PER,
        x label style={at={(axis description cs:0.5,0.025)},anchor=north},
        y label style={at={(axis description cs:0.1,.5)},anchor=south}
        ]
\addplot[color=blue] table[x=x,y=y] {dat/sweep.dat};

\addplot [name path=upper,draw=none] table[x=x,y expr=\thisrow{y}+\thisrow{err}] {dat/sweep.dat};
\addplot [name path=lower,draw=none] table[x=x,y expr=\thisrow{y}-\thisrow{err}] {dat/sweep.dat};
\addplot [fill=blue, fill opacity=0.5] fill between[of=upper and lower];

\addplot[color=black, dashed] table[x=x,y=y] {dat/big_only.dat};
% \addplot [name path=upper,draw=none] table[x=x,y expr=\thisrow{y}+\thisrow{err}] {dat/big_only.dat};
% \addplot [name path=lower,draw=none] table[x=x,y expr=\thisrow{y}-\thisrow{err}] {dat/big_only.dat};
% \addplot [fill=black, fill opacity=0.5] fill between[of=upper and lower];

\legend{,,,,Big network only};

\end{axis}
\end{tikzpicture}
    \caption{Test PER for Mini-LibriSpeech when increasing the controller bias.} % (The black dashed line represents the performance of the model which only uses the big network during both training and testing.)
    \label{fig:sweep}
\end{figure}

\clearpage
\section*{Appendix C: Effect of deterministic execution}

In our main experiments, the big network is selected stochastically with probability $p_{big}$, rather than deterministically when $p_{big}$ is greater than 0.5. This makes the comparison with randomized controllers in the ablation study more appropriate and removes the possibility of certain unlucky edge cases---for example, if $p_{big}$ is just barely less than 0.5 for the entirety of an input sequence, the big network would never be sampled in deterministic execution.

However, it is sometimes desirable for the execution of a model to be deterministic, e.g.~to make software testing easier and to obviate the need for random number generation when implementing the model in on a resource-limited device. We therefore also report the test results when the big network is selected deterministically in Tables \ref{det-ms} and \ref{det-timit}. It appears that when training stochastically, deterministic execution at test time causes a small increase in PER, though this is not reflected in the test loss. Also, it appears crucial to train stochastically, as otherwise overfitting occurs more easily, possibly because the big and small networks always see the same input observations.

\begin{table}[h]
% \centering
\caption{Results comparing deterministic and stochastic execution for Mini-LibriSpeech.}
\label{det-ms}
\begin{tabular}{cccccc}
\toprule
\thead{Stochastic\\ during training?} & \thead{Stochastic\\ during testing?} & \thead{Train loss} & \thead{Test loss} & \thead{Test PER} & \thead{Avg. FLOPs\\per input}\\
\midrule
\xmark & \xmark     & 69.96 $\pm$ 0.41 & 62.80 $\pm$ 0.76 &  26.45\% $\pm$ 0.23\% &  6.43M       \\ % 
\xmark  & \cmark  & 69.72  $\pm$ 0.43 &  63.69 $\pm$ 0.36 & 26.48\% $\pm$ 0.14\% &  6.43M    \\ % 
\cmark & \xmark  &  73.76  $\pm$ 0.31  & 62.15 $\pm$ 0.60 & 25.98\% $\pm$ 0.26\% &   6.43M    \\% 
\cmark & \cmark  &  74.30 $\pm$ 0.52  & 62.18 $\pm$ 0.64 & \textbf{25.80\%} $\pm$ 0.10\%  & 6.43M   \\  
\bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
% \centering
\caption{Results comparing deterministic and stochastic execution for TIMIT.}
\label{det-timit}
\begin{tabular}{cccccc}
\toprule
\thead{Stochastic\\ during training?} & \thead{Stochastic\\ during testing?} & \thead{Train loss} & \thead{Test loss} & \thead{Test PER} & \thead{Avg. FLOPs\\per input}\\
\midrule
\xmark & \xmark     & 16.19 $\pm$ 0.14  &  24.61 $\pm$ 0.52 &  21.00\% $\pm$ 0.19\%  &  6.41M       \\ % 
\xmark  & \cmark  & 16.21 $\pm$ 0.08 & 25.11 $\pm$ 0.24  & 20.81\% $\pm$ 0.24\% &  6.41M    \\ % 
\cmark & \xmark  &  17.58  $\pm$ 0.20 & 23.88 $\pm$ 0.31 & 20.08\% $\pm$ 0.22\% &   6.41M    \\% 
\cmark & \cmark  &  17.55 $\pm$ 0.26  &  24.04 $\pm$ 0.22  &  \textbf{20.00\%} $\pm$ 0.15\%   & 6.41M   \\  
\bottomrule
\end{tabular}
\end{table}

(It is possible to train a model either stochastically or deterministically, and then test it both stochastically and deterministically, thus avoiding redundant training runs. The train loss is only different between the first and second rows and between the third and fourth rows because it did not occur to us at the time of this experiment to implement this optimization.)

\clearpage
\section*{Appendix D: More detail on the learned controller baseline}

When comparing the performance of surprisal-based controllers with learned controllers in Section \ref{sec:compare}, we noted that the learned controllers' performance is sensitive to the hyperparameter $\lambda$ used in the loss function. This observation is illustrated for Mini-LibriSpeech in Figure \ref{fig:learnedcontroller}. 

Of course, this result should be taken with a grain of salt: the space of possible models for implementing the learned controller is vast, and there may be others that are more robust. Still, the fact that a gating network using the straight-through estimator---the simplest and best-performing approach to learned conditional computation considered in \cite{bengio2013estimating}---behaves this way suggests that other learned conditional computation methods, such as those based on reinforcement learning, may encounter similar difficulties.

\begin{figure}[h]
    \centering
\hspace*{-0.5cm} 
    \begin{tikzpicture}[font=\fontsize{7}{7}\selectfont]
\begin{axis}[
    % ytick={, 26.3},
        height=5.5cm,
        width=7cm,
        xmode = log,
        xmin=0.00001,
        xmax=0.1,
        ymin=25,
        ymax=36,
        every axis plot/.append style={thick},
        xlabel=$\lambda$,
        ylabel=PER,
        x label style={at={(axis description cs:0.5,0.025)},anchor=north},
        y label style={at={(axis description cs:0.1,.5)},anchor=south}
        ]
\addplot[color=red] table[x=x,y=y] {dat/learnedcontroller.dat};

\addplot [name path=upper,draw=none] table[x=x,y expr=\thisrow{y}+\thisrow{err}] {dat/learnedcontroller.dat};
\addplot [name path=lower,draw=none] table[x=x,y expr=\thisrow{y}-\thisrow{err}] {dat/learnedcontroller.dat};
\addplot [fill=red, fill opacity=0.5] fill between[of=upper and lower];

\addplot[color=black, dashed] table[x=x,y=y] {dat/randomcontroller.dat};
% \addplot [name path=upper,draw=none] table[x=x,y expr=\thisrow{y}+\thisrow{err}] {dat/big_only.dat};
% \addplot [name path=lower,draw=none] table[x=x,y expr=\thisrow{y}-\thisrow{err}] {dat/big_only.dat};
% \addplot [fill=black, fill opacity=0.5] fill between[of=upper and lower];

\addplot[color=blue, dashed] table[x=x,y=y] {dat/surprisalcontroller.dat};
% \addplot [name path=upper,draw=none] table[x=x,y expr=\thisrow{y}+\thisrow{err}] {dat/big_only.dat};
% \addplot [name path=lower,draw=none] table[x=x,y expr=\thisrow{y}-\thisrow{err}] {dat/big_only.dat};
% \addplot [fill=black, fill opacity=0.5] fill between[of=upper and lower];

\legend{,,,,Random controller,Surprisal-based controller};


\end{axis}
\end{tikzpicture}
    \caption{Test PER for Mini-LibriSpeech for models with a learned controller as a function of $\lambda$.}
    \label{fig:learnedcontroller}
\end{figure}
